Optimization in Open Networks via Dual Averaging

In networks of autonomous agents (e.g., fleets of vehicles, scattered sensors), the problem of minimizing the sum of the agents' local functions has received a lot of interest. We tackle here this distributed optimization problem in the case of open networks when agents can join and leave the network at any time. Leveraging recent online optimization techniques, we propose and analyze the convergence of a decentralized asynchronous optimization method for open networks.

==> Content/Deprecated/Deprecated-analysis.tex <==
\subsection{A more practical learning rate}

\FI{Copy paste below!}

Since the network of agents may be evolving, the average number of workers $\rms{\nWorkers}$ may often not be available in advance. A first solution can be taking learning rates of the form $\vwt[\step]=\vt[\step]=\Theta(1/\nWorkers_{\max}\sqrt{\delaybound\run})$. However, this still requires the knowledge of the global time\;$\run$ which is typically out of reach in the setup we are considering; in addition, it can be overly pessimistic with the dependence in $\nWorkers_{\max}\sqrt{\delaybound}$.
In order to get finer results, one needs to resort to adaptive parameters. For this, we need the following assumption concerning the feedback arrival on different nodes.

\begin{assumption}
\label{asm:card-in-order-global}
If $(\workeralt,\runalt)\in\vwt[\set]$ then $\card(\vwt[\set][\workeralt][\runalt])<\card(\vwt[\set])$.
\end{assumption}

This assumption simply means that if agent $\worker$ uses a feedback $\vwt[\gvec][\workeralt][\runalt]$ (\ie transmitted by agent $\workeralt$ ) at time $\run$, then agent $\worker$ has more gradients at time $\run$, than  agent $\workeralt$ at time $\runalt$.
Under this assumption, we show that it is possible for the agents to collaborate even if the average number of nodes and 
the time index $\run$ is not known by the agents.


\begin{theorem}
\label{thm:delay-regret-global-oblivious}
Let Assumptions \ref{asm:gen} and  \ref{asm:card-in-order-global} hold. 
Then, \eqref{eq:DDDA} with stepsizes
\begin{equation}
\label{eq:delay-global-oblivious-stepsize}
\vwt[\step]=\frac{\radius}{\gbound\sqrt{(5\delaybound+3)(\card(\vwt[\set])+(\delaybound+1)\nWorkers_{\max})\nWorkers_{\max}}}
\end{equation}
guarantees a bound on the running loss of
\begin{equation}
    \notag
    \runloss(\nRuns) = 
    \bigoh\left(\frac{\sqrt{\delaybound\nWorkers_{\max} \frac{1}{\nRuns}\sum_{\run=\start}^\nRuns\vt[\nWorkers]}}{\sqrt{\nRuns}}\right).
\end{equation}
\end{theorem}


\section{Asymptotic convergence}


\subsection{The case of fixed agents $\current[\Agents]=\Agents$}

In this particular case, we can define the (fixed) global loss as
\begin{align}
    \obj(\point) = \sum_{\worker\in\Agents} \vwup[\obj](\point).
\end{align}


We can apply Decentralized Dual Averaging with the constant stepsize
\[\vwt[\step]\equiv\step=\frac{\radius}{\gbound\nWorkers\sqrt{(2\delaybound+1)\nRuns}}\]
where $\nWorkers = \card(\Agents)$ is the number of agents.


Theorem~\ref{thm:delay-regret-global} then tells us that for any agent $\workeralt\in\Agents$:
%
\begin{align*}
 \obj\underbrace{\left( \frac{1}{\nRuns}\sum_{\run=\start}^{\nRuns}\vwt[\state][\run][\workeralt]\right)}_{\overline{\vwt[\state][\nRuns][\workeralt]}}
    - \min_{\comp\in\points} \obj(\comp) &\le
\frac{1}{\nRuns}\sum_{\run=\start}^{\nRuns} \obj(\vwt[\state][\run][\workeralt])
    - \min_{\comp\in\points} \obj(\comp) \\
    &\le \frac{    2\radius\gbound{\nWorkers}\sqrt{(2\delaybound+1)}}{\sqrt{\nRuns}}
.
\end{align*}


This means that the running average of the iterates at every agent guarantees a decrease in global suboptimality at rate $1/\sqrt{\nRuns}$.

\subsection{The case of recurring agents}

We now divide the agents $\Agents$ depending on their activity
\begin{align}
    \vw[\activity][\worker] \defeq \lim_{\nRuns\to\infty}\frac{\card\left( \run\leq\nRuns: \worker\in\current[\Agents]  \right)}{\nRuns}
\end{align}
into two categories: 
\begin{itemize}
    \item the recurring agents $\recAgents$ for which $\vw[\activity][\worker]>0 $;
    \item the transient agents $\transAgents$ for which $\vw[\activity][\worker] =0$.
\end{itemize}

==> Content/Deprecated/Deprecated-introduction.tex <==
Multi-agent systems are a powerful modeling framework for the analysis of signal processing or machine learning over sensor networks, fleets of autonomous vehicles, opi\-nion dynamics, etc. 
This framework calls for decentralized optimization methods where the agents seek to minimize the sum of the individual functions by exchanging information through a communication graph, without the help of a central authority. Indeed, such methods are key to perform distributed computing, signal processing, or learning from scattered sources in communication-constrained or large-scale environments; see e.g \cite{tsitsiklis1984problems,boyd2006randomized,dimakis2010gossip,lian2018asynchronous} and references therein. % \cite{tsitsiklis1984problems,boyd2006randomized,olfati2007consensus,dimakis2010gossip,lian2018asynchronous}


Hence, decentralized optimization methods have been extensively studied in the literature. Depending on the agents computing abilities and task at hand, several types of algorithms were considered. On the one hand, (sub-)gradient methods \cite{nedic2009distributed,bianchi2012convergence,jakovetic2014fast}, EXTRA \cite{shi2015extra},  DIGing \cite{nedic2017achieving}, and dual averaging \cite{duchi2011dual,tsianos2012push,lee2017stochastic,colin2016gossip} use (sub-)gradient of the agents' objective functions which is adapted to many situations of interest. % (see \cite{scaman2017optimal,kovalev2020optimal} for performance lower-bounds and a recent review). 
%Subgradient based methods such as ... use 
On the other hand, splitting methods such as the alternating direction method of multipliers (ADMM) \cite{boyd2011distributed,iutzeler2013asynchronous,wei20131} imply that each agents has to minimize (a regularized version of) its local function, which can be too demanding depending on the application. % \cite{boyd2011distributed,iutzeler2013asynchronous,wei20131,shi2014linear,iutzeler2015explicit}



An important aspect for scalability and flexibility of these methods is the possibility for asynchronous communications (\ie the agents do not synchronize to communicate between optimization steps) with delays (\ie there may be some gap between the sending time and the receiving time). The study of this aspect was thus concomitant to the development of the methods mentioned above; see \eg  \cite{tsianos2012consensus,wu2017decentralized,zhou2018distributed}. % \cite{agarwal2012distributed,tsianos2012consensus,wu2017decentralized,sirb2018decentralized,zhou2018distributed}.

%Open network: failure and deployment, elastic resource, vehicles

One common assumpton

In this paper, we focus on the particular case of asynchronous open networks where i) the agents can communicate with each other following a time-varying communication graph; ii) the exchanges and local processing incur delays; and iii) the agents may join and leave the system for arbitrary periods of time. While the first two points have been extensively studied in the literature as mentioned above, the last point tremendously complicates the analysis since the system may completely change from one step to another, see eg. \cite{de2020fundamental} and references therein.

\YGH{Add motivation for open systems + develop a bit more on contribution + reduce the number of references}


Due to the dynamic nature of these open multi-agents systems, several works have studied the stability of consensus algorithm over the mean, maximum, or median of the agents values \cite{Franceschelli2018proportional,Dashti2019dynamic,franceschelli2020stability,de2019lower,de2020open}. However, very few works tackle the problem of decentralized optimization over open networks. A notable exception is \cite{hendrickx2020stability} in which the authors show that decentralized gradient descent is stable when agents/functions change over time if their objectives are sufficiently smooth.



In this paper, we develop the idea that (offline) optimization problems over open networks can be efficiently handled by the tools from online optimization.
%treating them as online optimization algorithms.
Using this viewpoint and building on recent results on dual averaging for online learning with delays \cite{hsieh2020multi},
we introduce \acs{DAERON} (\acl{DAERON}), a method for optimization over open networks that allows for asynchronous communications.
\acused{DAERON}
On the theoretical side, we study the algorithm's performance averaged both across time and agents that are present in the network.
%with respect to the running average of the functions of agents present in the network.
We then provide numerical simulations on a decentralized regression problem to illustrate the potential of our method.
%we propose an asynchronous method for optimization over networks and study its performance with respect to the running average of the functions of agents present in the network. 

The rest of the paper is organized as follows.
In \cref{sec:framework}, we formulate the open multi-agent optimization problem mathematically and define the corresponding performance measures.
The main algorithm is described in \cref{sec:DAERON} and analyzed in \cref{sec:analysis}.
%, where we prove a $\bigoh(1/\sqrt{\nRuns})$ convergence rate for the considered measure.
%In \cref{sec:framework}, we introduce our open multi-agent framework and the corresponding performance measures. 
%In \cref{sec:framework}, we introduce our open multi-agent framework and the corresponding performance measures. 
%Then, we introduce our algorithm DAERON for Dual AvERaging for Open Network in Section~\ref{sec:DAERON} and analyze it in Section~\ref{sec:analysis}. Finally, we conduct some numerical experiments that justify our algorithmic choices in Section~\ref{sec:experiments}.
\cref{sec:experiments} is dedicated to numerical experiments.
Finally, \cref{sec:conclusion} concludes the paper and provides several clues for future research.

==> Optimization on Asynchronous Open Networks with Dual Averaging/Algos/DAERON.tex <==
\newcommand{\smallsim}{\smallsym{\mathrel}{\sim}}

\makeatletter
\newcommand{\smallsym}[2]{#1{\mathpalette\make@small@sym{#2}}}
\newcommand{\make@small@sym}[2]{%
  \vcenter{\hbox{$\m@th\downgrade@style#1#2$}}%
}
\newcommand{\downgrade@style}[1]{%
  \ifx#1\displaystyle\scriptstyle\else
    \ifx#1\textstyle\scriptstyle\else
      \scriptscriptstyle
  \fi\fi
}
\makeatother

\begin{algorithm}[tb]
    \caption{DAERON at node $\worker$ for active\;period\;$\jointime$-$\leavetime$}
    \label{algo:DAERON}
\begin{algorithmic}[1]
    \STATE {\bfseries Parameters:}
    $\jointime$ time when the agent joins the network;\\
    $\leavetime$ time when the agent leaves the network
    \STATE {\bfseries Initialize:}
         $\vwt[\set][\worker][\jointime] \subs \vwt[\set][\workeralt][\jointime]$ for $\workeralt\in\vt[\Agents][\jointime-1]\intersect\vt[\Agents][\jointime]$
    \FOR{$\run=\jointime,\ldots,\leavetime$}
    \STATE Generate the prediction $\vwt[\state]$ using \eqref{eq:DDDA}
    \STATE Compute the local subgradient $\vwt[\gvec]\in\subd\vw[\obj](\vwt[\state])$
    %\STATE // Possibly in parallel with lines $4-5$
    \STATE Send subgradients to other active agents
    %Send and receive subgradients 
    %\Comment{Possibly in parallel with lines $4-5$}
    %$\setdef{(\workeralt,\runalt)}{(\workeralt,\runalt)\in\vwt[\gvecs]}$
    \STATE Receive subgradients identified by the index set $\vwt[\gvecs]$
    \STATE Update $\vwtupdate[\set]\subs\vwt[\set]\union\vwt[\gvecs]\union\{\vwt[\gvec]\}$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Optimization on Asynchronous Open Networks with Dual Averaging/Algos/OpenNetwork.tex <==
\begin{algorithm}[tb]
    \caption{DAERON at each node $\worker$ as implemented in \cref{subsec:exp-open}}
    \label{algo:open-network}
\begin{algorithmic}[1]
    \STATE {\bfseries Initialize:}
         $\vwt[\set][\worker][\start] \subs \emptyset$, activation status $\vw[\activeStatus]\in\{0,1\}$, network parameters $K\in\N$, $p\in[0,1]$
    \FOR{$\run=\running$}
    \STATE \texttt{\underline{Agent update}}\\[0.1em]
    \IF{$\vw[\activeStatus]=1$}
    \STATE Get randomly paired with another active agent $\workeralt$
    \STATE Compute $\vwt[\state]$ by \eqref{eq:DDDA} and $\vwt[\gvec]\in\subd \vw[\obj](\vwt[\state])$
    \STATE Update $\vwtupdate[\set]\subs\vwt[\set]\union\vwt[\set][\workeralt]\union\{\vwt[\gvec]\}$
    %$\vt[\state] = \argmin_{\point\in\points} \sum_{\runalt\in\vt[\set]}\product{\vt[\gvec][\runalt]}{\point} + \frac{\norm{\point}^2}{2\vt[\step]}$
    \ENDIF
    \STATE \texttt{\underline{Network evolution}}\\[0.1em]
    \IF{$(\run+1)\equiv 0\mod K$}
    \STATE Draw a Bernoulli random variable $\vw[z]\sim\mathcal{B}(p)$
    \STATE $\vw[\activeStatus] \subs \vw[\activeStatus]+\vw[z]\mod 2$
    \IF{$\vw[z]=1$ and $\vw[\activeStatus] = 1$}
    \STATE Pick randomly $\workeralt \in \vt[\Agents]\intersect\vt[\Agents][\run+1]$
    \STATE Update $\vwtupdate[\set]\subs\vwtupdate[\set][\workeralt]$
    \ENDIF
    \ENDIF
    \ENDFOR
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
%     \caption{DARON at each node $\worker$}
%     \label{algo:adadelay-dist}
% \begin{algorithmic}[1]
%     \STATE {\bfseries Initialize:}
%         Gradient set $\vw[\set] \subs \emptyset$, stepsize $\step$
%     \FOR{$\run=\running$}
%     \IF{$\worker\in\vt[\Agents]$}
%     \STATE Get randomly paired with another active agent $\workeralt$
%     \STATE Compute $\vwt[\state]$ by \eqref{eq:DDDA} and $\vwt[\gvec]\in\subd \vw[\obj](\vwt[\state])$
%     \STATE Update $\vwtupdate[\set]\subs\vwt[\set]\union\vwt[\set][\workeralt]\union\{\vwt[\gvec]\}$
%     %$\vt[\state] = \argmin_{\point\in\points} \sum_{\runalt\in\vt[\set]}\product{\vt[\gvec][\runalt]}{\point} + \frac{\norm{\point}^2}{2\vt[\step]}$
%     \ENDIF
%     \ENDFOR
% \end{algorithmic}
% \end{algorithm}
 
% \begin{algorithm}[tb]
%     \caption{Open network evolution}
%     \label{algo:open-network}
% \begin{algorithmic}[1]
%     \STATE {\bfseries Initialize:}
%         Activation status $\vw[\activeStatus]\in\{0,1\}$
%     \FOR{$\run=\running$}
%     \IF{$\run\equiv 0\mod K$}
%     \STATE Draw a Bernoulli variable $\vw[z]\sim\mathcal{B}(p)$
%     \STATE $\vw[\activeStatus] \subs \vw[\activeStatus]+\vw[z]\mod 2$
%     \IF{$\vw[z]=1$ and $\vw[\activeStatus] = 1$}
%     \STATE Pick randomly $\workeralt \in \vt[\Agents][\run-1]\intersect\vt[\Agents]$
%     \STATE Update $\vwtupdate[\set]\subs\vwtupdate[\set][\workeralt]$
%     \ENDIF
%     \ENDIF
%     \ENDFOR
%  \end{algorithmic}
%  \end{algorithm}


==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Algorithm.tex <==
\input{Algos/DAERON}

\subsection{Algorithm}

\ac{DAERON}, as described in \cref{algo:DAERON}, is a (sub)gradient-based method that applies dual averaging \cite{Nes09} at the level of the whole network.
For this, we assume that given any point $\vwt[\point]\in\points$, the agent $\worker$ is able to compute a subgradient $\vwt[\gvec]\in\subd\vw[\obj](\vwt[\point])$.
This information is transmitted to the whole network and used by all the agents for computing their own variable.
Formally, let us define $\vwt[\set]$ as the index set of the subgradients that the agent $\worker\in\vt[\Agents]$ has received/computed by time $\run$.
Then, the agent $\worker$ generates the variable $\vwt[\state]$ as
%
%For the sake of simplicity, we also restrict ourselves to a model where the computations are immediate, \ie at each time slot $\run$, each active agent produces a prediction $\vwt[\state]$ and computes $\vwt[\gvec]\in\subd\vw[\obj](\vwt[\point])$.
%
%These assumptions allow us to give a simple description of \ac{DAERON} %as shown 
%in \cref{algo:DAERON}.
%Conceptually, each active agent $\worker\in\vt[\Agents]$ maintains a set of received/computed subgradients $\setdef{\vwt[\gvec][\workeralt][\runalt]}{(\workeralt,\runalt)\in\vwt[\set]}$ and generates the prediction $\vwt[\state]$ by %using a projection step
%
\begin{equation}
\label{eq:DDDA}
    \vwt[\state] = \proj_{\points} \left(
    \vt[\point][\start]
    -\vwt[\step]\!\sum_{(\workeralt,\runalt)\in\vwt[\set]}\vwt[\gvec][\workeralt][\runalt]
    \right).
\end{equation}
%
where $\proj_{\points}\from\dvec\mapsto\argmin_{\point\in\points}\norm{\point-\dvec}$ denotes the %Euclidean
projection onto $\points$, $\vt[\state][\start]$ is a common starting point, 
%and $\step>0$ is the stepsize of the algorithm.
and $\vwt[\step]>0$ is a learning rate that can be both time and agent dependent.
%Then, the nodes only need to exchange and accumulate all the subgradients that they have received or computed.
Note also that the communication of the subgradients (lines 6-7) can be done asynchronously in parallel with the other steps (lines 4-5) of the algorithm.

\begin{remark}[Arriving agents]
In \cref{algo:DAERON}, we initialize an agent arriving at time $\run$ with the subgradient set of an arbitrary agent in $\vt[\Agents][\run-1]\intersect\vt[\Agents]$, which implicitly assumes that $\vt[\Agents][\run-1]\intersect\vt[\Agents]\neq\emptyset$.
This is not crucial, as what really counts is that the agent is initialized with sufficient knowledge about what the network has computed, but we will stick to this model in the remainder of the paper for simplicity.
\end{remark}

% At time $\run$, an active agent $\agent\in\current[\Agents]$ performs successively three actions:
% \begin{itemize}
%     \item[1)] Compute a subgradient  on its local function. We denote this subgradient by  $\vwt[\gvec][\worker][\run-1] \in \partial \vwup[\obj][\worker](\vwt[\state][\worker][\run-1])$.
%     \item[2)] Send/Receive subgradients. We note $\vwt[\set]$ the set of  (agent, time) indices of available subgradients at time $\run$ for worker $\worker$, including its own.
%     \item[3)] Update. This is done by performing a decentralized dual averaging step:
% %     \begin{equation}
% % \label{eq:DDDA}
% %     \tag{DDA}
% %     \vwt[\state] = \argmin_{\point\in\points} \sum_{(\workeralt,\runalt)\in\vwt[\set]}\product{\vwt[\gvec][\workeralt][\runalt]}{\point} + \frac{\hreg(\point)}{\vwt[\step]},
% % \end{equation}
% with some stepsize $\vwt[\step]>0$.
% \end{itemize}

% Inactive agents lay dormant ($ \vwt[\state]= \vwt[\state][\agent][\run-1]$); the first time they are active, say $\runalt$, they are initialized with $\vwt[\state][\agent][\runalt-1]=\argmin_{\point\in\points}\hreg(\point) $.

\subsection{Practical Implementation}\label{sec:practical}

Storing all the available subgradients at a node can be prohibitively expensive, or even infeasible since this would require infinite storage capacity when $\run$ goes to infinity.
It is thus important to note that \ac{DAERON} is just a conceptual algorithm that can be implemented in different ways to circumvent this issue. %, depending on the problems that we have at hand.
We provide below two possible workarounds to demonstrate the flexibility of our method:

\begin{itemize}[leftmargin=5mm,itemsep=1mm]
    \item We can maintain $\vwt[\dvec]=\sum_{(\workeralt,\runalt)\in\vwt[\set]}\vwt[\gvec][\workeralt][\runalt]$ while keeping track of the most recent subgradients in order to communicate them with other agents.
    Formally, suppose that each node has a number of potential neighbors they may be connected to; then a subgradient $\vwt[\gvec][\workeralt][\runalt]$ only needs to be stored until the time that it has been sent to or received from these potential neighbors.
    % for each of the potential neighbors, $\vwt[\gvec][\workeralt][\runalt]$ has been sent to or received from that neighbor.
    %, either the node has sent $\vwt[\gvec][\workeralt][\runalt]$ to it, or the node has received $\vwt[\gvec][\workeralt][\runalt]$ from it, in which case it does not send $\vwt[\gvec][\workeralt][\runalt]$ back to the same neighbor.
    %they are communicated to all the potential neighbors (either the node sends $\vwt[\gvec][\workeralt][\runalt]$ to the neighbor or the node has received $\vwt[\gvec][\workeralt][\runalt]$ from a neighbor in which case it does not send it back to the same neighbor).
    
    \item If the number of involved agents $\nWorkers$ is small, we may define the sum of the subgradients computed by agent $\agent$ as  $\vwt[\agentsum]=\sum_{\runalt=1}^{\run-1}\vwt[\gvec][\worker][\runalt]$ with the convention $\vwt[\gvec][\worker][\runalt]=0$ when $\worker\notin\vt[\Agents][\runalt]$.
    Each node $\agent\in\vt[\Agents]$ then stores a table of size $\nWorkers\times\vdim$ containing the vectors $\vwt[\agentsum][1][\run-\delayij[\run][1]], \ldots, \vwt[\agentsum][\nWorkers][\run-\delayij[\run][\nWorkers]]$ corresponding to delayed versions of the computed subgradient sums over the network, with  $\delayij$ measuring this delay.
    %Here, $\delayij$ are delays indicating that the information about other nodes may not be up to date.
    These vectors are updated through communication. This strategy can also be adopted in a semi-centralized network with $\nWorkers$ central nodes and an arbitrary number of edge computing devices that retrieve information from these central nodes.
\end{itemize}

%While other heuristics that approximate the algorithm can also be considered, they may deprive us from the theoretical guarantee that we are going to provide in \cref{sec:analysis}.



\subsection{Quantities at play and assumptions}

For our analysis, we make the following technical assumptions on the local cost functions and the constraint set.

\vspace{2pt}
\begin{assumption}
\label{asm:cost}
Each $\vwup[\obj]$ is convex and $\gbound$-Lipschitz. The common constraint set $\points$ is closed and convex.
%All the loss functions $(\vwup[\obj])_{\worker\in\Agents}$ are convex and $\gbound$-Lipschitz for some $\gbound>0$.
\end{assumption}
\vspace{2pt}


In order for the problem to make sense, we will assume that the communication delays are upper bounded.
%Our assumption on the delays is crucial to the analysis.

\vspace{2pt}
\begin{assumption}
\label{asm:delay}
The delays of the algorithm are upper bounded %\footnote{With the notation of\;\ref{sec:practical}, this means $\delayij\le\delaybound$ for all $\worker$, $\workeralt$, and $\run$.} 
by $\delaybound$, \ie for any $\run,\runalt\in\N$ such that $\run>\runalt+\delaybound$ and any $\worker\in\vt[\Agents]$, $\workeralt\in\vt[\Agents][\runalt]$, we have $(\workeralt,\runalt)\in\vwt[\set]$.
\end{assumption}
\vspace{2pt}

In particular, \cref{asm:delay} supposes that every piece of information is spread to the whole network in a finite amount of time. While this is quite evident in a static network,
in the case of an open network this requires that the evolution of the network is slow enough with respect to the communication between the agents.


For concreteness, let us consider a model where every node communicates all its available gradients to its neighbors at each iteration. Then for a static network with a fixed topology $\graph=(\vertices,\edges)$, we have clearly $\delaybound=\diam(\graph)$ where $\diam(\graph)$ stands for the diameter of the graph.
The case of an open network with changing topology is considerably more complicated. For instance, in the case of a line graph where at each time a new agent joins at the end of the graph, the diameter grows linearly with $\run$ and it becomes impossible to propagate information to the whole network.
This is one kind of situation we want to avoid here.
Formally, we define $\vt[\Agents^{\workeralt,\runalt}]=\setdef{\worker\in\vt[\Agents]}{(\workeralt,\runalt)\in\vwt[\set]}$ as the set of active agents that possess $\vwt[\gvec][\workeralt][\runalt]$ at time $\run$.
The following example provides a sufficient stability assumption which allows information to spread across the network.

\begin{example}[Bounded delays]
\label{ex:vertex-connected}
Come back to the same situation as above where every node communicates all its available gradients to its neighbors during each iteration. Suppose further that the set of the active agents remain unchanged for periods of $\evolveInt$ iterations (\ie for $\run=\runano\evolveInt,\ldots,(\runano+1)\evolveInt-1$), and that the graph $\graph_\runano=(\vt[\vertices],\Union_{\run=\runano\evolveInt}^{\runano(\evolveInt+1)-1}\vt[\edges][\runalt])$ is $\connectivity$-vertex-connected (\ie removing at least $\connectivity$ nodes is necessary to disconnect it).
If the number of arriving plus leaving agents at the end of iteration $(\runano+1)\evolveInt-1$ is $\nChange<\connectivity$, then for any $\runalt\leq\runano\evolveInt-1$ and $\workeralt\in\vt[\Agents][\runalt]$, the number of nodes that do not possess $\vwt[\gvec][\workeralt][\runalt]$ is reduced by at least $\connectivity-\nChange>0$ after the $\evolveInt$ iterations, \ie $\card(\vt[\Agents^{\workeralt,\runalt}][(\runano+1)\evolveInt])\le\max(0,\card(\vt[\Agents^{\workeralt,\runalt}][\runano\evolveInt])-(\connectivity-\nChange))$.
%the number of nodes that do not possess $\vwt[\gvec][\worker][\runalt]$ ($\runalt\leq\runano\evolveInt$) is reduced by at least $\connectivity-\nChange>0$. 
In that case, the maximal delay is thus bounded by $\max_\run \vt[\nWorkers]\evolveInt/( \connectivity-\nChange)+\evolveInt$. % we can add a -1 in both m and B, i.e., (m-1)/(k-q)+B-1
\end{example}

The above example means that provided that the number of exiting/incoming agents is not too large compared to the connectivity of the communication graph, the delays are naturally bounded.


\begin{remark}[Loss of information due to agent departure]
When an agent leaves the network,
%at time $\leavetime$, 
some of its computed subgradients may be lost for the network.
%, say those between $\losttime$ and $\leavetime$.
This can happen either because it never communicated them or because the agents to which it communicated them also left the network.
In \cref{ex:vertex-connected}, the change of composition at the end of iteration $(\runano+1)\evolveInt-1$ could notably cause the loss of the subgradients computed at time $\run=\runano\evolveInt,\ldots,(\runano+1)\evolveInt-1$.
%the loss of information can notably happens to the subgradients computed between 
This does not affect the proposed algorithm. The only difference is in the analysis: we will consider that the agent $\workeralt$ is not in $\current[\Agents][\runalt]$ if $\vt[\Agents^{\workeralt,\runalt}]=\emptyset$ starting from some $\run$.\footnote{%
Note that in \cref{ex:vertex-connected}, we have either $\vt[\Agents^{\workeralt,\runalt}]=\emptyset$ or $\vt[\Agents^{\workeralt,\runalt}]=\vt[\Agents]$ for $\run$ sufficiently large (assuming that $\runalt$ is fixed).
}
%for all $\run\geq\losttime$, as if it actually left the network at $\losttime$.
\end{remark}


% We provide the following proposition to illustrate the idea that the evolution of the network need.
% We assume that all the nodes that leave the network communicate their subgradients to another node before departure (otherwise a subgradient may disappear from the network and we will need to modify the definition of $\runloss$ to accommodate it).



% \vspace{2pt}
% \begin{proposition}
% Suppose that the set of the active agents remain unchanged for $\evolveInt$ iterations $\runalt=\run,\ldots,\run+\evolveInt-1$,
% %\ie $\vt[\Agents][\run]=\ldots=\vt[\Agents][\run+\evolveInt-1]$
% and that the graph $\graph=(\vt[\vertices],\Union_{\runalt=\run}^{\run+\evolveInt-1}\vt[\edges][\runalt])$ is $\connectivity$-vertex-connected.
% Then, if the number of arriving plus leaving agents at the end of iteration $\run+\evolveInt-1$ is $\nChange<\connectivity$,
% %(\ie $\card(\setexclude{\vt[\Agents][\run+\evolveInt]}{\vt[\Agents][\run+\evolveInt-1]})+\card(\setexclude{\vt[\Agents][\run+\evolveInt-1]}{\vt[\Agents][\run+\evolveInt]})=\nChange$)
% for any $\vwt[\gvec][\worker][\runalt]$ with $\runalt<\run$,
% the number of nodes that do not possess $\vwt[\gvec][\worker][\runalt]$ is reduced by at least $\connectivity-\nChange$ until it gets spread to the whole network after the $\evolveInt$ iterations.
% \end{proposition}
% \vspace{2pt}

% \begin{itemize}
% \item $\delaybound$ (explain the communications and link with $\current[\Edges]$)
% \item $\radius$ such that $\hreg(\comp^\star)\le\radius^2$,
% \end{itemize}



==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Analysis.tex <==
\subsection{Performance in the general case}

We provide the convergence result for \ac{DAERON} in terms of the running loss defined in \eqref{eq:running-loss}. To do so, we define the quadratic mean and the average number of active agents over time:

\begin{equation}
    \notag
    \rms{\nWorkers}=\sqrt{\frac{1}{\nRuns}\sum_{\run=\start}^\nRuns\vt[\nWorkers^2]}
    \quad\text{and}\quad
    \avg[\nWorkers]=\frac{1}{\nRuns}\sum_{\run=\start}^\nRuns\vt[\nWorkers].
\end{equation}
Note that we always have $\rms{\nWorkers}\ge\avg[\nWorkers]$.
% $\rms{\nWorkers}=\sqrt{(1/\nRuns)\sum_{\run=\start}^\nRuns\vt[\nWorkers^2]}$ and $\avg[\nWorkers]=(1/\nRuns)\sum_{\run=\start}^\nRuns\vt[\nWorkers]$ 
%respectively for the \ac{RMS} number and the average number of active agents over time.

%The (root mean square) average number of active agents by $\rms{\nWorkers}=\sqrt{(1/\nRuns)\sum_{\run=\start}^\nRuns\vt[\nWorkers]^2}$ and the maximum number of active agents by $\nWorkers_{\max}=\max_{\start\le\run\le\nRuns}\vt[\nWorkers]$ will obviously play a role in the subsequent analysis.

\vspace*{1ex}
\begin{theorem}
\label{thm:delay-regret-global}
Let \cref{asm:cost,asm:delay} hold.
Running \ac{DAERON} with constant learning rate
\begin{equation}
    \notag
    \vwt[\step]\equiv
    \step
    =
    \frac{\smallradius_0}{\rms{\nWorkers}\gbound\sqrt{(3\delaybound+1)\nRuns}}
\end{equation}
for some $\smallradius_0>0$ guarantees that %the following convergence rate on the running loss:
%
\begin{equation}
    \label{eq:regret-fixed-lr}
    \runloss(\nRuns)
    \le \frac{\rms{\nWorkers}}{\avg[\nWorkers]}
    \frac{2\regcst\smallradius\gbound\sqrt{3\delaybound+1}}{\sqrt{\nRuns}},
\end{equation}
where $\smallradius=\norm{\sol[\comp]-\vt[\state][\start]}^2$ and
$\regcst=\max(\smallradius/(2\smallradius_0), \smallradius_0/\smallradius)$.
\end{theorem}





\begin{proof}
\input{Content/Proof}
\end{proof}

\cref{thm:delay-regret-global} shows that when the ratio $\rms{\nWorkers}/\avg[\nWorkers]$ is upper bounded, the running loss of the algorithm has a convergence rate in $\bigoh(1/\sqrt{\nRuns})$.
% \FI{It is always upper bounded by $1$ and lower bounded by $1/\sqrt{T}$ no?}
% %if the learning rate is suitably chosen.
% This is notably the case when $\vt[\nWorkers]$ is upper bounded or grows linearly.
The factor $\rms{\nWorkers}/\avg[\nWorkers]$ also indicates that the algorithm converges slower when the number of active agents varies greatly across iterations,
which is expected because the algorithm would need more time to accommodate the change in this situation.

\begin{remark}[Extensions]
One drawback of the theorem is that the expression of the learning rate involves both the sqaure mean number of the agents $\rms{\nWorkers}$ and the time horizon $\nRuns$.
In a continuously evolving network, neither of these two quantities are known in advance.
%the RMS number of the agents $\rms{\nWorkers}$ nor the time horizon $\nRuns$ should be known in advance.
We provide below several alternatives which allow us to establish the same $\bigoh(1/\sqrt{\nRuns})$ rate without these quantities. Proofs are variations of the above proof; we omit details due to space limitations. 
\begin{itemize}[leftmargin=5mm,itemsep=1mm]
    \item If the number $\vt[\nWorkers]$ is known to every agent.
    %of agents that are presented in the network at each time instant is a shared knowledge.
    We may use $\vwt[\step]=\vt[\step]=\Theta(1/\sqrt{\delaybound(\sum_{\runalt=1}^{\run}\vt[\nWorkers^2][\runalt])})$.
    \item If $\nWorkers_{\max}=\max_{1\le\run\le\nRuns}\vt[\nWorkers]$ can be estimated and the agents have access to a global clock that indicates $\run$, we can take $\vwt[\step]=\vt[\step]=\Theta(1/(\nWorkers_{\max}\sqrt{\delaybound\run}))$.
    \item Note that $\sqrt{\sum_{\runalt=1}^{\run}\vt[\nWorkers^2][\runalt]}\le\sqrt{\nWorkers_{\max}}\sqrt{\vt[\nWorkersSum]}$.
    Therefore, provided that $\nWorkers_{\max}$ is known, another alternative is to use $\vwt[\step]=\Theta(1/\sqrt{\delaybound\nWorkers_{\max}\vt[\nWorkersSum]})$. This does not require to know $\vt[\nWorkers]$ explicitly since $\vt[\nWorkersSum]$ can be estimated by $\card(\vwt[\set])$. In particular, under \cref{asm:delay}, it holds $\vt[\nWorkersSum]\le\card(\vwt[\set])+(\delaybound+1)\nWorkers_{\max}$.
    % One plausible solution is to replace $\rms{\nWorkers}$ by a running average or the maximum number of agents that can be presented in the network $\nWorkers_{\max}=\max_{1\le\run\le\nRuns}\vt[\nWorkers]$ and take $\vwt[\step]=\vt[\step]=\Theta(1/\nWorkers_{\max}\sqrt{\delaybound\run})$.
% If the agents do not have access to a global clock, we can also estimate $\vt[\nWorkersSum]$ by $\card(\vwt[\set])$ and use $\rms{\nWorkers}\le\sqrt{\nWorkers_{\max}\avg[\nWorkers]}$.
\medskip
\end{itemize}
\end{remark}



\subsection{The case of fixed agents $\current[\Agents]=\Agents$}

For comparison with existing literature (\eg \cite{duchi2011dual}), we now turn back to the case of a ``closed network'' where all the agents are active at each iteration.
In this situation, we can define the (fixed) global loss as
\begin{equation}
    \notag
    \obj(\point) = \frac{1}{\nWorkers} \sum_{\worker\in\Agents} \vwup[\obj](\point),
\end{equation}
where $\nWorkers = \card(\Agents)$ is the number of agents. We have $\rms{\nWorkers}=\avg[\nWorkers]=\nWorkers$ and thus $\rms{\nWorkers}/\avg[\nWorkers]=1$.
As an immediate corollary of \cref{thm:delay-regret-global}, if we apply \ac{DAERON} with the constant stepsize
%We can apply Decentralized Dual Averaging with the constant stepsize
\[\vwt[\step]\equiv\step=\frac{\smallradius}{\nWorkers\gbound\sqrt{(3\delaybound+1)\nRuns}},\]
then for any  agent $\worker\in\Agents$, 
%Theorem~\ref{thm:delay-regret-global} then tells us that for any agent $\workeralt\in\Agents$:
%
\begin{align*}
 \obj
 %\underbrace{
 \left( \frac{1}{\nRuns}\sum_{\run=\start}^{\nRuns}\vwt[\state]\right)%}
 %_{\overline{\vwt[\state]}}
    - \min_{\comp\in\points} \obj(\comp) &\le
\frac{1}{\nRuns}\sum_{\run=\start}^{\nRuns} \obj(\vwt[\state])
    - \min_{\comp\in\points} \obj(\comp) \\%[-3ex]
    &\le \frac{    2\smallradius\gbound\sqrt{3\delaybound+1}}{\sqrt{\nRuns}}
.
\end{align*}
This means
%a $\bigoh(1/\sqrt{\nRuns})$ convergence rate in global suboptimality for the running average of each agent's iterates,
that the running average of each agent's iterates decreases in global suboptimality at rate $\bigoh(1/\sqrt{\nRuns})$,
which matches the rate of \cite[Th.~2]{duchi2011dual} for the slightly different decentralized dual averaging algorithm.\footnote{In \cite{duchi2011dual}, the subgradient are averaged by gossiping while in  \ac{DAERON}, they are directly exchanged.}
Going one step further, the same result would still hold under asynchronous activation as long as the activation patterns can be described by a stationary probability distribution. 
On the other hand, \cref{thm:delay-regret-global} also allows us to prove the convergence of the algorithm in an open network whose composition stops changing after finite time.
%We omit the detailed descriptions of these results here due to space limitations.
%With similar techniques, from \cref{thm:delay-regret-global} we can also derive (asymptotic) convergence rate for an open network whose composition stops changing after finite time or a closed network with asynchronous activation if the activation patterns are described by a fixed probability distribution. 
%(\ie only a random set of agents are active at each $\run$) or an open network whose composition would stop changing after a finite of time.

% \subsection{The case of recurring agents}

% We now divide the agents $\Agents$ depending on their activity
% \begin{align}
%     \vw[\activity][\worker] \defeq \lim_{\nRuns\to\infty}\frac{\card\left( \run\leq\nRuns: \worker\in\current[\Agents]  \right)}{\nRuns}
% \end{align}
% into two categories: 
% \begin{itemize}
%     \item the recurring agents $\recAgents$ for which $\vw[\activity][\worker]>0 $;
%     \item the transient agents $\transAgents$ for which $\vw[\activity][\worker] =0$.
% \end{itemize}

% %\vspace{4pt}
% %\noindent
% \subsection*{Online to batch conversion}

% Let us now consider a setting where the functions $\vt[\instObj]$ can be modeled as random variables such that for a certain underlying function $\obj$ and a sequence of positive numbers $\seqinf[\vt[\scalar]]$, we have $\exof{\vt[\instObj]\given{\vt[\filter]}}=\vt[\scalar]\obj$ where $\seqinf[\vt[\filter]]$ is the natural filtration associated to $\seqinf[\vt[\instObj]]$.
% Then, applying the online to batch conversion \needref we get immediately that
% %
% \begin{equation}
% \begin{multlined}[b]
%     \ex\left[
%     \obj\left(\frac{\sum_{\run=1}^{\nRuns}\vt[\nWorkers]\vt[\scalar]\vt[\state^{\text{ref}}]}
%     {\sum_{\run=1}^{\nRuns}\vt[\nWorkers]\vt[\scalar]}\right)
%     \right] - \min_{\point\in\points}\obj(\point)
%     \\\le
%     \frac{\vt[\nWorkersSum][\nRuns]}{\sum_{\run=1}^{\nRuns}\vt[\nWorkers]\vt[\scalar]}
%     \ex\left[\runloss(\nRuns)\right]
% \end{multlined}
% \end{equation}

% \YGH{to complete}

==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Conclusion.tex <==
In this paper, we introduced a decentralized optimization method for open multi-agent systems, in which agents can freely join or leave the network during the process.
This setting is particularly challenging since there is not a clear objective to minimize and even exact convergence to a consensus is generally out of reach.
These difficulties led us to adopting techniques and performance measures from online optimization.
We proved that our algorithm benefits from a $\bigoh(1/\sqrt{\nRuns})$ convergence rate with respect to the running average of the functions of the agents present in the network. 
In our simulations, we showed that our method outperformed decentralized subgradient descent on a least absolute deviation problem.

The positive results in our numerical experiments also opens up several new research directions: To analyze the tracking behavior, it could be more relevant to focus on the dynamic regret \cite{HW15,SJ17} or to adopt the perspective of time-varying optimization \cite{Simonetto17,DSSM20}.
The goal here is either to bound the sum of the instantaneous optimality gaps or to show that the realized actions is always close to the current optimum.
%This would provide us a better understanding on the instantaneous performance of the algorithm.
Another promising direction is to explore the potential combination of \ac{DAERON} and consensus-based methods, which may lead to superior performance.
Given the variety of problems and open networks that we are facing, it is clear that there is not a single method that would outperform all the others. It is thus also important to find the most suitable algorithm for each specific setup.
%Finally, important to determine what is the best algorithm to use given a specific open network.

%also raises several important questions:
%How can we analyze the tracking behavior of the algorithm from a theoretical perspective?
%Is it possible to combine \ac{DAERON} with other consensus-based methods to achieve superior performance?
%How do we determine the best algorithm to use given a specific open network?
%Each of these question leads to new research direction that is worth exploring in future works.


%As shown in the experiments, a constant learning rate may equip the algorithm with the capacity to track the instantaneous solution
%adhoc algorithms for specific settings

==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Deprecated/Deprecated-analysis.tex <==
\subsection{A more practical learning rate}

\FI{Copy paste below!}

Since the network of agents may be evolving, the average number of workers $\rms{\nWorkers}$ may often not be available in advance. A first solution can be taking learning rates of the form $\vwt[\step]=\vt[\step]=\Theta(1/\nWorkers_{\max}\sqrt{\delaybound\run})$. However, this still requires the knowledge of the global time\;$\run$ which is typically out of reach in the setup we are considering; in addition, it can be overly pessimistic with the dependence in $\nWorkers_{\max}\sqrt{\delaybound}$.
In order to get finer results, one needs to resort to adaptive parameters. For this, we need the following assumption concerning the feedback arrival on different nodes.

\begin{assumption}
\label{asm:card-in-order-global}
If $(\workeralt,\runalt)\in\vwt[\set]$ then $\card(\vwt[\set][\workeralt][\runalt])<\card(\vwt[\set])$.
\end{assumption}

This assumption simply means that if agent $\worker$ uses a feedback $\vwt[\gvec][\workeralt][\runalt]$ (\ie transmitted by agent $\workeralt$ ) at time $\run$, then agent $\worker$ has more gradients at time $\run$, than  agent $\workeralt$ at time $\runalt$.
Under this assumption, we show that it is possible for the agents to collaborate even if the average number of nodes and 
the time index $\run$ is not known by the agents.


\begin{theorem}
\label{thm:delay-regret-global-oblivious}
Let Assumptions \ref{asm:gen} and  \ref{asm:card-in-order-global} hold. 
Then, \eqref{eq:DDDA} with stepsizes
\begin{equation}
\label{eq:delay-global-oblivious-stepsize}
\vwt[\step]=\frac{\radius}{\gbound\sqrt{(5\delaybound+3)(\card(\vwt[\set])+(\delaybound+1)\nWorkers_{\max})\nWorkers_{\max}}}
\end{equation}
guarantees a bound on the running loss of
\begin{equation}
    \notag
    \runloss(\nRuns) = 
    \bigoh\left(\frac{\sqrt{\delaybound\nWorkers_{\max} \frac{1}{\nRuns}\sum_{\run=\start}^\nRuns\vt[\nWorkers]}}{\sqrt{\nRuns}}\right).
\end{equation}
\end{theorem}


\section{Asymptotic convergence}


\subsection{The case of fixed agents $\current[\Agents]=\Agents$}

In this particular case, we can define the (fixed) global loss as
\begin{align}
    \obj(\point) = \sum_{\worker\in\Agents} \vwup[\obj](\point).
\end{align}


We can apply Decentralized Dual Averaging with the constant stepsize
\[\vwt[\step]\equiv\step=\frac{\radius}{\gbound\nWorkers\sqrt{(2\delaybound+1)\nRuns}}\]
where $\nWorkers = \card(\Agents)$ is the number of agents.


Theorem~\ref{thm:delay-regret-global} then tells us that for any agent $\workeralt\in\Agents$:
%
\begin{align*}
 \obj\underbrace{\left( \frac{1}{\nRuns}\sum_{\run=\start}^{\nRuns}\vwt[\state][\run][\workeralt]\right)}_{\overline{\vwt[\state][\nRuns][\workeralt]}}
    - \min_{\comp\in\points} \obj(\comp) &\le
\frac{1}{\nRuns}\sum_{\run=\start}^{\nRuns} \obj(\vwt[\state][\run][\workeralt])
    - \min_{\comp\in\points} \obj(\comp) \\
    &\le \frac{    2\radius\gbound{\nWorkers}\sqrt{(2\delaybound+1)}}{\sqrt{\nRuns}}
.
\end{align*}


This means that the running average of the iterates at every agent guarantees a decrease in global suboptimality at rate $1/\sqrt{\nRuns}$.

\subsection{The case of recurring agents}

We now divide the agents $\Agents$ depending on their activity
\begin{align}
    \vw[\activity][\worker] \defeq \lim_{\nRuns\to\infty}\frac{\card\left( \run\leq\nRuns: \worker\in\current[\Agents]  \right)}{\nRuns}
\end{align}
into two categories: 
\begin{itemize}
    \item the recurring agents $\recAgents$ for which $\vw[\activity][\worker]>0 $;
    \item the transient agents $\transAgents$ for which $\vw[\activity][\worker] =0$.
\end{itemize}

==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Deprecated/Deprecated-introduction.tex <==
Multi-agent systems are a powerful modeling framework for the analysis of signal processing or machine learning over sensor networks, fleets of autonomous vehicles, opi\-nion dynamics, etc. 
This framework calls for decentralized optimization methods where the agents seek to minimize the sum of the individual functions by exchanging information through a communication graph, without the help of a central authority. Indeed, such methods are key to perform distributed computing, signal processing, or learning from scattered sources in communication-constrained or large-scale environments; see e.g \cite{tsitsiklis1984problems,boyd2006randomized,dimakis2010gossip,lian2018asynchronous} and references therein. % \cite{tsitsiklis1984problems,boyd2006randomized,olfati2007consensus,dimakis2010gossip,lian2018asynchronous}


Hence, decentralized optimization methods have been extensively studied in the literature. Depending on the agents computing abilities and task at hand, several types of algorithms were considered. On the one hand, (sub-)gradient methods \cite{nedic2009distributed,bianchi2012convergence,jakovetic2014fast}, EXTRA \cite{shi2015extra},  DIGing \cite{nedic2017achieving}, and dual averaging \cite{duchi2011dual,tsianos2012push,lee2017stochastic,colin2016gossip} use (sub-)gradient of the agents' objective functions which is adapted to many situations of interest. % (see \cite{scaman2017optimal,kovalev2020optimal} for performance lower-bounds and a recent review). 
%Subgradient based methods such as ... use 
On the other hand, splitting methods such as the alternating direction method of multipliers (ADMM) \cite{boyd2011distributed,iutzeler2013asynchronous,wei20131} imply that each agents has to minimize (a regularized version of) its local function, which can be too demanding depending on the application. % \cite{boyd2011distributed,iutzeler2013asynchronous,wei20131,shi2014linear,iutzeler2015explicit}



An important aspect for scalability and flexibility of these methods is the possibility for asynchronous communications (\ie the agents do not synchronize to communicate between optimization steps) with delays (\ie there may be some gap between the sending time and the receiving time). The study of this aspect was thus concomitant to the development of the methods mentioned above; see \eg  \cite{tsianos2012consensus,wu2017decentralized,zhou2018distributed}. % \cite{agarwal2012distributed,tsianos2012consensus,wu2017decentralized,sirb2018decentralized,zhou2018distributed}.

%Open network: failure and deployment, elastic resource, vehicles

One common assumpton

In this paper, we focus on the particular case of asynchronous open networks where i) the agents can communicate with each other following a time-varying communication graph; ii) the exchanges and local processing incur delays; and iii) the agents may join and leave the system for arbitrary periods of time. While the first two points have been extensively studied in the literature as mentioned above, the last point tremendously complicates the analysis since the system may completely change from one step to another, see eg. \cite{de2020fundamental} and references therein.

\YGH{Add motivation for open systems + develop a bit more on contribution + reduce the number of references}


Due to the dynamic nature of these open multi-agents systems, several works have studied the stability of consensus algorithm over the mean, maximum, or median of the agents values \cite{Franceschelli2018proportional,Dashti2019dynamic,franceschelli2020stability,de2019lower,de2020open}. However, very few works tackle the problem of decentralized optimization over open networks. A notable exception is \cite{hendrickx2020stability} in which the authors show that decentralized gradient descent is stable when agents/functions change over time if their objectives are sufficiently smooth.



In this paper, we develop the idea that (offline) optimization problems over open networks can be efficiently handled by the tools from online optimization.
%treating them as online optimization algorithms.
Using this viewpoint and building on recent results on dual averaging for online learning with delays \cite{hsieh2020multi},
we introduce \acs{DAERON} (\acl{DAERON}), a method for optimization over open networks that allows for asynchronous communications.
\acused{DAERON}
On the theoretical side, we study the algorithm's performance averaged both across time and agents that are present in the network.
%with respect to the running average of the functions of agents present in the network.
We then provide numerical simulations on a decentralized regression problem to illustrate the potential of our method.
%we propose an asynchronous method for optimization over networks and study its performance with respect to the running average of the functions of agents present in the network. 

The rest of the paper is organized as follows.
In \cref{sec:framework}, we formulate the open multi-agent optimization problem mathematically and define the corresponding performance measures.
The main algorithm is described in \cref{sec:DAERON} and analyzed in \cref{sec:analysis}.
%, where we prove a $\bigoh(1/\sqrt{\nRuns})$ convergence rate for the considered measure.
%In \cref{sec:framework}, we introduce our open multi-agent framework and the corresponding performance measures. 
%In \cref{sec:framework}, we introduce our open multi-agent framework and the corresponding performance measures. 
%Then, we introduce our algorithm DAERON for Dual AvERaging for Open Network in Section~\ref{sec:DAERON} and analyze it in Section~\ref{sec:analysis}. Finally, we conduct some numerical experiments that justify our algorithmic choices in Section~\ref{sec:experiments}.
\cref{sec:experiments} is dedicated to numerical experiments.
Finally, \cref{sec:conclusion} concludes the paper and provides several clues for future research.

==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Experiments.tex <==
In this section, we demonstrate the effectiveness of \ac{DAERON} with experiments on a static and an open network.

\subsection{Problem Description}

Let us consider a decentralized \ac{LAD} regression model.
Given a data set evenly distributed on $\nWorkers$ nodes $(\expvar_{\worker\indg},\resvar_{\worker\indg})_{\worker,\indg\in\oneto{\nWorkers}\times\oneto{\nSamplesPerWorker}}$ with $\expvar_{\worker\indg}$ in $\vecspace$ and $\resvar_{\worker\indg}\in\R$, it consists in solving 
%
\begin{equation}
    \label{eq:LAD}
    \min_{\point\in\vecspace}
    \left\{\obj(\point)\defeq
    \frac{1}{\nWorkers}\sumworker\frac{1}{\nSamplesPerWorker}\sum_{\indg=1}^\nSamplesPerWorker \abs{\expvar_{\worker\indg}^{\top}\point-\resvar_{\worker\indg}}\right\}.
\end{equation}
%
Compared to least square regression, \ac{LAD} is known to be more resistant to the presence of outliers. 
%Moreover, the non-differentiability of the problem makes the use of subgradients necessary and would thus uses the full generality of our method. (to be rephrased)
Although the use of absolute value makes the problem non-differentiable, \ac{DAERON} can be run with subgradients as suggested by our analysis.
%but the optimum can still be found by performing 
%For simplicity, we assume that the data are evenly distributed on $\nWorkers$ nodes, each of them possessing $\nSamplesPerWorker$ samples.
For the experiments, we generate synthetic data as follows:
\begin{enumerate}
    \item The ground truth model $\groundtruth\in[-5,5]^{\vdim}$ is drawn from a uniform distribution.
    \item The local model $\vw[\groundtruth]$ of the node $\worker$ is obtained by perturbing $\groundtruth$ with a Gaussian noise, \ie $\vw[\groundtruth]=\groundtruth+\vw[\varepsilon]$ where $\vw[\epsilon]\sim\mathcal{N}(0,\Id_{\vdim})$.
    \item We sample $\expvar_{\worker\indg}\sim\mathcal{N}(0,\Id_{\vdim})$ and compute $\resvar_{\worker\indg} = \expvar_{\worker\indg}^{\top}\vw[\groundtruth]+\varepsilon_{\worker\indg}$ with $\varepsilon_{\worker\indg}\sim\mathcal{N}(0,1)$.
    \item On each node, a random portion of samples are corrupted. For these samples, we replace $\resvar_{\worker\indg}$ by a random value generated from a Gaussian distribution.
\end{enumerate}
In the above, we introduce the second and the fourth steps mainly for two reasons. First, it makes the problem more heterogeneous, and thus more difficult. Second, it makes the communication between agents more important for finding a good approximation of $\groundtruth$.
In the following, we will take $\nWorkers=64$ nodes, $\nSamplesPerWorker=200$ samples per node, and dimension  $\vdim=20$.
On each node, the number of corrupted samples is random in $\intinterval{0}{120}$. We also verify that the solution $\expsol$ of \eqref{eq:LAD} is not too far from $\groundtruth$.

\input{Algos/OpenNetwork}

\subsection{Static network}

We first investigate the performance of the algorithm on a static network.
The nodes are arranged in a $2$d grid of size $8\times8$.
Adjacent nodes exchange gradients at each iteration.
%Each computed subgradient is broadcasted to the whole network, but a message can only travel from one node to its immediate neighbors at each time slot.
%\FI{I don't get the sentence above}
%During each iteration, each node computes a subgradient and relays all the subgradients that it just received (or computed) and had never seen before to its neighbors. 
Communication-computation overlap is allowed for better efficiency--- in \cref{algo:DAERON}, this means that lines 4-5 and 6-7 are run in parallel.
%occur at the same time.
Then, with a constant stepsize $\step$, the update writes
%
\begin{equation}
    \notag
    \vwtupdate[\state] = \vwt[\state] - \step \sumworker \vwt[\gvec][\workeralt][\run-\delay_{\workeralt,\worker}],
\end{equation}
%
where $\delay_{\workeralt,\worker}$ is the distance between the nodes $\workeralt$ and $\worker$.
For illustration purposes, we also compare with a \ac{DGD} method \cite{nedic2009distributed} with constant stepsize\;$\stepalt$ and a mixing matrix $\mixing=(\mixingw_{\worker,\workeralt})$. Its update is
%
\begin{equation}
    \notag
    \vwtupdate[\state] = \sum_{\workeralt=1}^{\nWorkers}\mixingw_{\worker,\workeralt}\vwt[\state][\workeralt] - \stepalt \vwt[\gvec]
\end{equation}
%
and we take $\mixing$ as the Metropolis matrix of the graph in our experiments:
%
\begin{equation}
    \notag
    \mixingw_{\worker,\workeralt}
    = \left\{
        \begin{array}{ll}
            1/(\max(\degr(\worker),\degr(\workeralt))+1) & \text{if } \{\worker,\workeralt\}\in\edges,\\
            1 - \sum_{\indg=1}^{\nWorkers}\mixingw_{\worker,\indg} & \text{if } \worker=\workeralt,\\
            0 & \text{otherwise},
        \end{array}
        \right.
\end{equation}
%
with $\degr(\worker)$ denoting the degree of the node $\worker$.

For a proper comparison of the two algorithms, it is important to notice that a subgradient is sent to all the $\nWorkers$ nodes in \name while it is averaged out in \ac{DGD}.
Therefore, we will take $\stepalt=\nWorkers\step$ and refer to it as the \emph{effective learning rate} of both methods.
With this in mind, in \cref{subfig:convergence-static-network} we plot the convergence of the averaged optimality gap $(1/\nWorkers)\sumworker\obj(\vwt[\state])-\min\obj$ for \ac{DAERON} and \ac{DGD} with different choices of $\stepalt$.

Interestingly, we observe that when using the same effective learning rate, the two algorithms establish similar convergence behavior until reaching their respective fixed points. However, \ac{DAERON} is able to converge to a point with higher accuracy.
We believe that this is because the variables $(\vwt[\state])_{\worker\in\Agents}$ tend to be closer to each other in \ac{DAERON}.\footnote{Indeed, let $\Delta$ and $1-\lambda$ be respectively the diameter of the graph and the spectral gap of the mixing matrix.
Then, as shown in the proof of \cref{thm:delay-regret-global}, for \ac{DAERON} we can roughly bound $\norm{\vwt[\state]-\vwt[\state][\workeralt]}$ by $\nWorkers\step\delaybound\gbound=\Delta\stepalt\gbound$.
As for \ac{DGD}, it is known that we have asymptotically $\norm{\vwt[\state]-\vwt[\state][\workeralt]}\lesssim\gamma\gbound/(1-\lambda)$ \cite[Lem.~11]{NOR18}.
Since it generally holds $\Delta\le1/(1-\lambda)$ and this is notably the case for the graph that we consider, this provides a possible explanation for the superiority of \ac{DAERON} over \ac{DGD}.}
%\footnote{%
%More precisely, we have $\Delta\lesssim1/\sqrt{1-\lambda}$ for many simple networks.}

%Further investigation shows that for a same effective learning rate, the primal variables $(\vwt[\state])$ get closer to each other for \ac{DAERON}


\input{Figures/Static+Open}

\subsection{Open network}
\label{subsec:exp-open}

Now that we have shown that \ac{DAERON} performs comparably to standard decentralized optimization methods in a static network, we proceed to study its behavior in an open multi-agent system (\cref{algo:open-network}).
%Our experimental setup along with the algorithm is summarized in \cref{algo:open-network}.
Following \cite{VMN18}, we model the arrivals and departures of the agents by a Bernoulli process.
Initially, only half of the $64$ nodes are active. Then, every $K=20$ iterations, each agent may change its activation status (\ie from active to inactive or vice-versa) with probability $p=0.05$.
At each iteration, the active nodes are randomly paired with each other, then each pair synchronizes their gradients.\footnote{%
If there is an odd number of nodes, one node is ignored in this process.}
%\FI{I changed the sentence above, is it ok?}
%\footnote{In practice, this does not require all the gradients to be stored physically and can be achieved with finite memory.}
Formally, if nodes $\worker$ and $\workeralt$ are paired at time $\run$, then 
%
%\begin{equation}
%    \notag
$
    \setexclude{\vwtupdate[\set]}{\{\vwt[\gvec]\}} = \setexclude{\vwtupdate[\set][\workeralt]}{\{\vwt[\gvec][\workeralt]\}}
    =\vwt[\set]\union\vwt[\set][\workeralt].
$
%\end{equation}
%
%An agent that becomes active at time $\run$ is assigned the gradient set of a random node in $\vt[\Agents][\run-1]\intersect\vt[\Agents]$.
%For the sake of clarity, the above is summarized as pseudo-code in \cref{algo:open-network}.
%Inspired by consensus-based methods, we also consider an algorithm where each agent maintains a local variable $\vwt[\state]$ and for any two agents $\worker$, $\workeralt$ that communicate at round $\run$, we have $\vwtupdate[\state]=(\vwt[\state]+\vwt[\state][\workeralt])-\stepalt\vwt[\gvec]$ and $\vwtupdate[\state][\workeralt]=(\vwt[\state]+\vwt[\state][\workeralt])-\stepalt\vwt[\gvec][\workeralt]$.
In the spirit of \ac{DGD}, we also implement an algorithm which directly updates the primal variables as
%such that if two agents $\worker$, $\workeralt$ communicate during round $\run$, we update
%
\begin{equation}
%\vwtupdate[\state]+\stepalt\vwt[\gvec]=\vwtupdate[\state][\workeralt]+\stepalt\vwt[\gvec][\workeralt]=\frac{\vwt[\state]+\vwt[\state][\workeralt]}{2}.
    \notag
    \begin{aligned}
    \vwtupdate[\state]&=\frac{\vwt[\state]+\vwt[\state][\workeralt]}{2}-\stepalt\vwt[\gvec],\\
    \vwtupdate[\state][\workeralt]&=\frac{\vwt[\state]+\vwt[\state][\workeralt]}{2}-\stepalt\vwt[\gvec][\workeralt].
    \end{aligned}
\end{equation}
%
In both cases, an agent that becomes active at the end of round $\run-1$ is assigned the state variable (\ie $\vwt[\set]$ or $\vwt[\state]$) of a random node in $\vt[\Agents][\run-1]\intersect\vt[\Agents]$.
We take $\stepalt=\nWorkers\step/2$ in our experiment since on average $\nWorkers/2$ nodes are active.% at each time instant.

As for the performance measure, we consider the averaged instantaneous optimality gap $\avgInstLoss(\run)$ and the averaged running loss $\avgRunLoss(\run)$ defined by
%In \cref{subfig:convergence-open-network} we plot both the averaged instantaneous optimality gap $\avgInstLoss(\run)$ and the averaged running loss $\avgRunLoss(\run)$ of the two algorithms defined by
%
\begin{align}
\avgInstLoss(\run)
&=
\frac{1}{\vt[\nWorkers]}\sum_{\worker\in\vt[\Agents]}\vt[\obj^{\text{inst}}](\vwt[\state])-\min\vtp[\obj]
\label{eq:avg-inst-loss}
\\
\avgRunLoss(\run)
&=
\frac{1}{\vt[\nWorkersSum]}
\sum_{\runalt=1}^{\run}
%\frac{1}{\vt[\nWorkers][\runalt]}
\sum_{\worker\in\vt[\Agents][\runalt]}\vt[\obj^{\text{inst}}][\runalt](\vwt[\state][\worker][\runalt])
-\min\vt[\obj^{\text{run}}].
\label{eq:avg-run-loss}
\end{align}
%
The evolution of these two measures for $\stepalt=0.005$ are plotted in \cref{subfig:convergence-open-network}.\footnote{This is roughly the largest stepsize that leads to the decrease of the losses.
We observe similar convergence patterns for smaller stepsizes, while the performance gap between the two algorithm diminishes.}
We see that both algorithms are able to converge to an area where potential solutions are located whereas \ac{DAERON} can get much closer to the optimum of $\vt[\instObj]$.
Moreover, we observe that the instantaneous loss for \ac{DAERON} increases abruptly when the set of active agents changes and gets decreased again afterwards.
This indicates that the algorithm actually has the ability to track the instantaneous solution.
%We believe that understanding this behavior from a theoretical perspective would be an important future direction to pursue.
%It would be interesting to study this behavior from a theoretical point of view.

%is actually tracking the solution. Similar phenomenon can also be observed for DGD when using a smaller learning rate, but this also implies slower adaption to the changing environment compared to DAERON
%While similar phenomenon should happen to DGD, the change in instantaneous objective is too small with respect to the optimality gap which makes it 

==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Framework.tex <==
\subsection{Model}

We consider a (possibly infinite) set of agents $\Agents$; each of them associated with an individual convex cost function $\vwup[\obj]\from \vecspace\to \R$. At each time $\run=\running$, only a (finite) subset of agents $\current[\Agents]$ is active and may communicate using undirected communications links $\current[\Edges] \defeq \{ \{\agent,\agentalt\}\in\current[\Agents]^2 : \agent \text{ and } \agentalt \text{ can exchange at } \run \}$.
%To avoid trivialities, we assume that $\vt[\Agents]\neq\emptyset$ for all $\run$.
Let $\vt[\nWorkers]\defeq\card(\vt[\Agents])$ denote the number of active agents at time $\run$ and we will also write $\vt[\nWorkersSum]\defeq\sum_{\runalt=\start}^{\run}\vt[\nWorkers][\runalt]$.
%and $\vt[\mmax{\nWorkers}]=\max_{1\le\run\le\nRuns}\vt[\nWorkers]$.
%and $\vt[\nWorkersSum]=\sum_{\runalt=\start}^{\run}\vt[\nWorkers][\runalt]$ denote respectively the number of agents at time $\run$ and accumulated over a horizon of $\run$ time steps.

%Each agent $\agent\in\Agents$ possess a convex lower semi-continuous function $\vwup[\obj]: \vecspace\to \R$ that typically represents the personal loss at agent $\agent$ and a common constraint set $\points$.

%We are interested in the problem of finding minimizing a global loss function that is defined as the average over 

In open multi-agent systems, it is in general impossible to define a temporally invariant global objective to minimize over time.
Since those who are present in the network are usually the entities that we really care about, an alternative is to focus exclusively on the active agents and define the instantaneous loss at time $\run$ as
%In order to minimize the loss over all active agents, the system would ideally like to minimize the instantaneous loss at each time $\run$, ie. 
\begin{align}
    \notag
    %\label{eq:inst-loss}
    %\min_{\point\in\points}
    %\left\{
        \vt[\obj^{\text{inst}}](\point)
        =\frac{1}{\vt[\nWorkers]}\sum_{\agent\in\current[\Agents]} \vwup[\obj](\point).
    %\right\}.
\end{align}
%However, such an objective is unrealistic since i) the set of active agents $\current[\Agents]$ can change drastically between two consecutive time instants
%arbitrarily which changes the objective over time; and ii) even agreeing on a consensus value in an open network is a difficult problem.
The problem of interest is then the minimization of $\vt[\obj^{\text{inst}}]$.
However, providing a proper analysis for this time-varying problem is still challenging because
the set of active agents $\current[\Agents]$ may change drastically between two consecutive time instants, which also leads to an abrupt change in the objective. In addition, agreeing on a consensus value in an open network is already a difficult problem \cite{franceschelli2020stability, de2020open}.


\subsection{Quantity of Interest}

Instead of tackling the minimization of $\vt[\obj^{\text{inst}}]$ directly, we draw inspiration from online learning and analyze the \emph{running loss} defined for a time-horizon $\nRuns$ as 
\begin{align}
    \label{eq:running-loss}
    \runloss(\nRuns)\!=\!\frac{1}{\vt[\nWorkersSum][\nRuns]}
    \!\!\left(
      \sum_{\run=\start}^{\nRuns}\!\sum_{\worker\in\current[\Agents]} \vwup[\obj](\vt[\state^{\text{ref}}])
    - \min_{\comp\in\points} \!\sum_{\run=\start}^{\nRuns}\!\sum_{\worker\in\current[\Agents]} \!\vwup[\obj](\comp)\!
    \right)
\end{align}
where $\points\subset\vecspace$ is the shared constrained set and $\vt[\state^{\text{ref}}]$ is a reference point for time $\run$. In the sequel, we will consider algorithms in which each agent $\worker\in\vt[\Agents]$ produces a local variable $\vwt[\state]$ at time $\run$. It is thus reasonable to set $\vt[\state^{\text{ref}}]=\vwtATt[\state]$ for a reference agent $\vt[\worker]\in\vt[\Agents]$ that is chosen arbitrarily at each time, and $\runloss$ would then represent the average network suboptimality over time for these reference agents.
%for the reference agents $\vt[\worker]\in\vt[\Agents]$ (chosen arbitrarily at each time). 
Note that the suboptimality is compared with the best fixed {\em a posteriori} action which is the solution $\sol[\comp]\in\points$ of
\begin{align}
    \notag
   \min_{\comp\in\points}
   \left\{
   \vt[\obj^{\text{run}}][\nRuns](\comp)
   \defeq
   \frac{1}{\vt[\nWorkersSum][\nRuns]}
   \sum_{\run=\start}^{\nRuns}\sum_{\worker\in\current[\Agents]} \vwup[\obj](\comp)
   \right\}.
\end{align}

This quantity mimics the collective regret in \cite{hsieh2020multi} with an additional $1/\vt[\nWorkersSum][\nRuns]$ which takes into account the total number of agents that have participated until time $\nRuns$. The notable difference here with the distributed online optimization literature \cite{HCM13,SJ17,YSVQ12} is that we consider an open network of agents so that the composition of the system can change over time.
%is that the agents' functions do not change over time; instead we aim at providing better bounds and algorithms for an open network of agents with fixed objective functions.
%The online nature of the problem is just a subproduct of the dynamics of the system.

% This formulation is typically suited for wireless sensor networks performing distributed estimation \cite{RN04} or data fusion \cite{NLF07,RCMP+15}.
% \FI{I kind of copy pasted above from JMLR, to reformulate}


% Indeed, sensor networks are often deployed to perform a global objective for which they cooperate. The notion of running loss then measure each agent's loss over the network and over time to capture how well it performs over the global task at hand.



==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Introduction.tex <==
Multi-agent systems are a powerful modeling framework for the analysis of signal processing or machine learning over sensor networks, fleets of autonomous vehicles, opi\-nion dynamics, etc. 
This framework calls for decentralized optimization methods where the agents seek to minimize the sum of the individual functions by exchanging information through a communication graph, without the help of a central authority. Indeed, such methods are key to perform distributed computing, signal processing, or learning from scattered sources in communication-constrained or large-scale environments; see e.g \cite{tsitsiklis1984problems,boyd2006randomized,dimakis2010gossip,lian2018asynchronous} and references therein. % \cite{tsitsiklis1984problems,boyd2006randomized,olfati2007consensus,dimakis2010gossip,lian2018asynchronous}


In this regard, decentralized optimization methods have been extensively studied in the literature. Depending on the agents' computing abilities and tasks at hand, several types of algorithms were considered. On the one hand, gradient-based methods such as decentralized gradient descent \cite{nedic2009distributed,bianchi2012convergence,jakovetic2014fast}, and decentralized dual averaging \cite{duchi2011dual,tsianos2012push,lee2017stochastic,colin2016gossip} update the local variables using gradients of the agents' objective functions (see also \cite{NOR18} for a recent review).
% (see \cite{scaman2017optimal,kovalev2020optimal} for performance lower-bounds and a recent review). 
%Subgradient based methods such as ... use 
On the other hand, splitting methods such as the alternating direction method of multipliers (ADMM) \cite{boyd2011distributed,iutzeler2013asynchronous,wei20131} imply that each agents has to minimize (a regularized version of) its local function, which can be too demanding depending on the application. % \cite{boyd2011distributed,iutzeler2013asynchronous,wei20131,shi2014linear,iutzeler2015explicit}

Despite the abundance of literature on this topic, most of them assume a network of fixed composition, that is, the agents that participate in the process always remain the same.
On the contrary, this work focuses on the case of an \emph{open network} where the agents can join and leave the system at any moment.
This can happen in numerous situations, \eg % for which we provide only a few examples below:

\begin{itemize}[leftmargin=5mm,itemsep=1mm]
    \item When a cluster of servers is used to train a machine learning task, a node may leave the network due to a system failure or simply because the resource is acquired by another job.
    %On the other hand,
    New nodes can also be deployed to accelerate the training process or process additional data.
    \item We can also think of the case of volunteer computing where volunteers provide computing resources for a distributed task. The network is naturally open since a device is only involved when the volunteer desires to participate.
    \item In multi-vehicle coordination, the set of vehicles that are considered by the algorithm can evolve with time.
\end{itemize}

Due to the dynamic nature of these open multi-agent systems, several works have studied the stability of consensus algorithm over the mean, maximum, or median of the agents values \cite{Franceschelli2018proportional,Dashti2019dynamic,franceschelli2020stability,de2019lower,de2020open}.
Among the very few works that tackle the problem of decentralized optimization over open networks,  \cite{hendrickx2020stability} showed that decentralized gradient descent is stable when agents/functions change over time if their objectives are sufficiently smooth.

%In parallel, <--- Maybe this is a pun, but it adds too much confusion! 
Distributed algorithms also need to cope with asynchronous communications (\ie the agents do not synchronize to communicate between optimization steps) with delays (\ie there may be some gap between sending and receiving times).
Such capacity is an important feature for scalability and flexibility.
The study of this aspect was thus concomitant to the development of different decentralized optimization methods; see \eg \cite{tsianos2012consensus,wu2017decentralized,zhou2018distributed}. % \cite{agarwal2012distributed,tsianos2012consensus,wu2017decentralized,sirb2018decentralized,zhou2018distributed}.

In this paper, we focus on the particular case of asynchronous open networks where i) the agents can communicate with each other asynchronously following a time-varying communication graph; ii) the exchanges and local processing incur delays; and iii) the agents may join and leave the system for arbitrary periods of time. While the first two points are relatively well studied in the literature as mentioned above (see also \cite{BKR19} for an online distributed algorithm with local processing delays), the last point tremendously complicates the analysis since the system may completely change from one step to another, see \eg \cite{de2020fundamental} and references therein.

To address this challenge, we develop the idea that (offline) optimization problems over open networks can be efficiently handled by tools from \emph{online optimization}.
%treating them as online optimization algorithms.
Using this viewpoint and building on recent results on dual averaging for online learning with delays \cite{hsieh2020multi},
we introduce \acs{DAERON} (\acl{DAERON}), a method for optimization over open networks that allows for asynchronous communications.
\acused{DAERON}
On the theoretical side, we study the algorithm's performance %averaged both across time and agents that are present in the network.
with respect to the average (over both time and agents) of the agents' functions.
We then provide numerical simulations on a decentralized regression problem to illustrate the potential of our method.
%we propose an asynchronous method for optimization over networks and study its performance with respect to the running average of the functions of agents present in the network. 

The rest of the paper is organized as follows.
In \cref{sec:framework}, we formulate the open multi-agent optimization problem mathematically and define the corresponding performance measures.
The main algorithm is described in \cref{sec:DAERON} and analyzed in \cref{sec:analysis}.
%, where we prove a $\bigoh(1/\sqrt{\nRuns})$ convergence rate for the considered measure.
%In \cref{sec:framework}, we introduce our open multi-agent framework and the corresponding performance measures. 
%In \cref{sec:framework}, we introduce our open multi-agent framework and the corresponding performance measures. 
%Then, we introduce our algorithm DAERON for Dual AvERaging for Open Network in Section~\ref{sec:DAERON} and analyze it in Section~\ref{sec:analysis}. Finally, we conduct some numerical experiments that justify our algorithmic choices in Section~\ref{sec:experiments}.
\cref{sec:experiments} is dedicated to numerical experiments.
Finally, \cref{sec:conclusion} concludes the paper and provides several clues for future research.

==> Optimization on Asynchronous Open Networks with Dual Averaging/Content/Proof.tex <==
An important feature of \name is that the subgradients are not always applied to the points where they are evaluated.
To accommodate this in our analysis, we consider the virtual iterates $\seqinf[\vt[\virtual]]$ defined by
%
\begin{equation}
    \notag
    \vt[\virtual] = \proj_{\points}\left(\vt[\state][\start]-
    \step\sum_{\run=\start}^{\run-1}\sum_{\worker\in\vt[\Agents]}\vwt[\gvec]\right).
\end{equation}

From the regret analysis of dual averaging (see, \eg \cite[Prop. 2]{DHS11}), the following holds for all $\comp\in\points$,
%
\begin{equation}
    \notag
    \begin{aligned}[b]
    \sum_{\run=1}\sum_{\worker\in\vt[\Agents]}
    \product{\vwt[\gvec]}{\vt[\virtual]-\comp}
    &\le
    \frac{\norm{\comp-\vt[\state][\start]}^2}{2\step}
    +\frac{\step}{2}\sum_{\run=1}^{\nRuns}
    \bigg\|\sum_{\worker\in\vt[\Agents]}\vwt[\gvec]\bigg\|^2\\
    &\le
    \frac{\norm{\comp-\vt[\state][\start]}^2}{2\step}
    +\frac{\step}{2}\sum_{\run=1}^{\nRuns}\vt[\nWorkers^2]\gbound^2.
    \end{aligned}
\end{equation}
%
In the second line we have used the Lipschitz continuity of the functions which implies that $\norm{\vwt[\gvec]}\le\gbound$.
Next, by using the convexity and the Lipschitz continuity of the functions, each term of \eqref{eq:running-loss} can be bounded for any $\comp\in\points$ by
%
\begin{align}
    \notag
    \vw[\obj](\vt[\state^{\text{ref}}]) - \vw[\obj](\comp)
    &= \vw[\obj](\vwtATt[\state]) - \vw[\obj](\vwt[\state])
    + \vw[\obj](\vwt[\state]) - \vw[\obj](\comp)\\
    \notag
    &\le \gbound\norm{\vwtATt[\state]-\vwt[\state]}
    + \product{\vwt[\gvec]}{\vwt[\state]-\comp}.
\end{align}
%
We proceed to bound the second term in the above inequality
%
\begin{equation}
    \notag
    \begin{aligned}[b]
    \product{\vwt[\gvec]}{\vwt[\state]-\comp}
    &= \product{\vwt[\gvec]}{\vwt[\state]-\vt[\virtual]}
    + \product{\vwt[\gvec]}{\vt[\virtual]-\comp}\\
    &\le \gbound\norm{\vwt[\state]-\vt[\virtual]}
    + \product{\vwt[\gvec]}{\vt[\virtual]-\comp}.
    \end{aligned}
\end{equation}
%
Using the triangle inequality, we get $\norm{\vwtATt[\state]-\vwt[\state]}\le\norm{\vwtATt[\state]-\vt[\virtual]}+\norm{\vwt[\state]-\vt[\virtual]}$.
Now, let $\vt[\Gamma] = \max_{\worker\in\vt[\Agents]}\norm{\vwt[\state]-\vt[\virtual]}$ and set $\comp\subs\sol[\comp]$. We have from the above
%
\begin{equation}
    \notag
    \runloss(\nRuns)
    \le \frac{1}{\vt[\nWorkersSum]}
    \left(
    \frac{\norm{\sol[\comp]-\vt[\state][\start]}^2}{2\step}
    +\sum_{\run=1}^{\nRuns}
    (\frac{\step}{2}\vt[\nWorkers^2]\gbound^2
    +3\vt[\nWorkers]\gbound\vt[\Gamma])
    \right).
\end{equation}

To conclude, we may bound $\vt[\Gamma]$ thanks to the bounded delay assumption.
In fact, since the projection operator is non-expansive, it holds for all $\worker\in\vt[\Agents]$ that 
%
\begin{equation}
    \notag
    \addtocounter{footnote}{-1}
    \begin{multlined}
    \norm{\vwt[\state]-\vt[\virtual]}
    \le \bigg\|
    \step\sum_{\run=\start}^{\run-1}
    \sum_{\workeralt\in\vt[\Agents]}\vwt[\gvec]
    - 
    \step\sum_{(\workeralt,\runalt)\in\vwt[\set]}\vwt[\gvec][\workeralt][\runalt]
    \bigg\| \\
    \le \bigg\|
    \step\sum_{\runalt=\run-\delaybound}^{\run-1}
    \sum_{\workeralt\in\vt[\Agents][\runalt]}\vwt[\gvec][\workeralt][\runalt]
    \bigg\|
    \le \step\sum_{\runalt=\run-\delaybound}^{\run-1} \vt[\nWorkers][\runalt]\gbound.\footnotemark
    \end{multlined}
    \footnotetext{If $\runalt\le0$, then $\vt[\Agents][\runalt]=\emptyset$ and $\vt[\nWorkers]=0$.}
\end{equation}
%
Then, with $\vt[\nWorkers]\vt[\nWorkers][\runalt]\le(\vt[\nWorkers^2]+\vt[\nWorkers^2][\runalt])/2$, we obtain the following
%
\begin{equation}
    \notag
    \runloss(\nRuns)
    \le \frac{1}{\vt[\nWorkersSum]}
    \left(
    \frac{\norm{\sol[\comp]-\vt[\state][\start]}^2}{2\step}
    +\step\gbound^2\sum_{\run=1}^{\nRuns}
    (3\delaybound+1)\vt[\nWorkers^2]
    \right).
\end{equation}
Inequality \eqref{eq:regret-fixed-lr} follows immediately by the definition of $\rms{\nWorkers}$, $\avg[\nWorkers]$, and $\regcst$.

==> Optimization on Asynchronous Open Networks with Dual Averaging/Figures/Static+Open.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/StaticNetwork_Losses.pdf}
    \caption{Static network}
    \label{subfig:convergence-static-network}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/OpenNetwork_Losses.pdf}
    \caption{Open network}
    \label{subfig:convergence-open-network}
    \end{subfigure}
    \caption{Comparison of \ac{DAERON} and \ac{DGD}.
    For a static network we plot in (a) the averaged suboptimality. For an open network we plot in (b)
    the averaged instantaneous suboptimality \eqref{eq:avg-inst-loss} and the averaged running loss \eqref{eq:avg-run-loss}.}
    \label{fig:convergence}
\end{figure}
